Understanding and Bridging the Modality Gap for Speech Translation

How to achieve better end-to-end speech translation (ST) by leveraging (text) machine translation (MT) data? Among various existing techniques, multi-task learning is one of the effective ways to share knowledge between ST and MT in which additional MT data can help to learn source-to-target mapping. However, due to the differences between speech and text, there is always a gap between ST and MT. In this paper, we first aim to understand this modality gap from the target-side representation differences, and link the modality gap to another well-known problem in neural machine translation: exposure bias. We find that the modality gap is relatively small during training except for some difficult cases, but keeps increasing during inference due to the cascading effect. To address these problems, we propose the Cross-modal Regularization with Scheduled Sampling (Cress) method. Specifically, we regularize the output predictions of ST and MT, whose target-side contexts are derived by sampling between ground truth words and self-generated words with a varying probability. Furthermore, we introduce token-level adaptive training which assigns different training weights to target tokens to handle difficult cases with large modality gaps. Experiments and analysis show that our approach effectively bridges the modality gap, and achieves promising results in all eight directions of the MuST-C dataset.

==> Figures/figure_three_minipage.tex <==
\begin{figure}
  \begin{minipage}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Figure_heatmap.pdf}
    \caption{The heat map of BLEU scores with different combinations of $B$ (base) and $S$ (scale) for \textbf{\textsc{Cress+}}. The BLEU score of \textbf{\textsc{Cress}} is 28.0.}
    \label{fig:heatmap}
  \end{minipage}
  \begin{minipage}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Figure_modality_gap_cmp.pdf}
    \caption{Curves of the average modality gap with decoding steps under three strategies. The dotted line refers to \textbf{\textsc{MTL}} (same as Figure \ref{fig:exposure_bias}), and the solid line refers to \textbf{\textsc{CRESS+}}.}
    \label{fig:modality_gap_cmp}
  \end{minipage}
  \begin{minipage}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Figure_bleu_sentence_length.pdf}
    \caption{BLEU scores at different target sentence lengths.}
    \label{fig:bleu_sentence_length}
  \end{minipage}
\end{figure}

==> Figures/figure_two_minipage.tex <==
\begin{figure}
  \begin{minipage}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Figure_cos_dist_cmp.pdf}
    \caption{Distributions of the modality gap on MuST-C En$\rightarrow$De \texttt{dev} set of \textbf{\textsc{MTL}} and \textbf{\textsc{Cress}} with kernel density estimation (KDE).}
    \label{fig:cos_dist_cmp}
  \end{minipage}
  \hspace{0.04\linewidth}
  \begin{minipage}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Figure_modality_gap_cmp.pdf}
    \caption{Curves of the average modality gap with decoding steps under three strategies. The dotted line refers to \textbf{\textsc{MTL}} (same as Figure \ref{fig:exposure_bias}), and the solid line refers to \textbf{\textsc{CRESS}}.}
    \label{fig:modality_gap_cmp}
  \end{minipage}
\end{figure}

==> Figures/figure_two_minipage_ii.tex <==
\begin{figure}
  \begin{minipage}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Figure_heatmap.pdf}
    \caption{The heat map of BLEU scores on MuST-C En$\rightarrow$De \texttt{dev} set with different combinations of $B$ and $S$. The BLEU score without token-level adaptive training is 28.0.}
    \label{fig:heatmap}
  \end{minipage}
  \hspace{0.04\linewidth}
  \begin{minipage}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Figure_bleu_sentence_length.pdf}
    \caption{BLEU scores on MuST-C En$\rightarrow$De \texttt{dev} set at different target sentence lengths.}
    \label{fig:bleu_sentence_length}
  \end{minipage}
\end{figure}

==> Sections/D00_impact_of_decay_parameter.tex <==
\label{sec:decay}
In scheduled sampling, the probability of selecting the ground truth word $p^*$ keeps decreasing during training as the function in Equation (\ref{eq:decay}). Here, the hyper-parameter $\mu$ is used to control the shape of the function. As $\mu$ increases, the probability $p^*$ decreases more slowly, and vice versa. We investigate the impact of $\mu$ in Figure \ref{fig:decay}, and find that (1) the model performs worse when $p^*$ drops too quickly, and (2) when $\mu$ is within a reasonable range, there is not much impact on the final BLEU score. We use $\mu=15$ in our experiments.
\input{Figures/figure_decay}

==> Sections/F00_mt_performance.tex <==
Since our method is built upon the multi-task learning framework, we also report the performance of the MT task. As shown in Table \ref{tab:mt}, our method not only brings improvements to ST, but also gives a slight average boost of 0.3 BLEU to MT. We suggest that this may be due to the effect of regularization. More importantly, we find that the performance gap between ST and MT for \textbf{\textsc{Cress}} is significantly reduced compared to the \textbf{\textsc{MTL}} baseline (6.0$\rightarrow$5.0), which further demonstrates that the improvement in ST is mainly due to the effective reduction of the modality gap.

\input{Tables/table_mt}

==> Sections/H00_base_and_scale.tex <==
\label{sec:basescale}
$B$ (base) and $S$ (scale) are two important hyper-parameters in token-level adaptive training. We investigate how different combinations of $B$ and $S$ influence performance. As shown in Figure \ref{fig:heatmap}, token-level adaptive training can bring improvements in most cases. In particular, it usually performs better with smaller $B$ and smaller $S$, leading to a boost of up to 0.4 BLEU. We conclude that treating different tokens too differently is also undesirable. We use $B=0.7$ and $S=0.05$ for all translation directions.
\input{Figures/figure_heatmap}
